The Outburst of the Blazar AO 0235+164 in 2006 December: Shock-in-Jet Interpretation

We present the results of polarimetric ($R$ band) and multicolor photometric ($BVRIJHK$) observations of the blazar AO 0235+16 during an outburst in 2006 December. The data reveal a short timescale of variability (several hours), which increases from optical to near-IR wavelengths; even shorter variations are detected in polarization. The flux density correlates with the degree of polarization, and at maximum degree of polarization the electric vector tends to align with the parsec-scale jet direction. We find that a variable component with a steady power-law spectral energy distribution and very high optical polarization (30-50%) is responsible for the variability. We interpret these properties of the blazar withina model of a transverse shock propagating down the jet. In this case a small change in the viewing angle of the jet, by $\lesssim 1^o$, and a decrease in the shocked plasma compression by a factor of $\sim$1.5 are sufficient to account for the variability.

==> table1.tex <==
\begin{deluxetable}{lrlrlrlr}
\singlespace
\tablecolumns{8}
\tablecaption{\bf Optical Data \label{TAB_1}}
\tabletypesize{\footnotesize}
\tablehead{
\colhead{MJD}&\colhead{$B$}&\colhead{MJD}&\colhead{$V$}&
\colhead{MJD}&\colhead{$R$}&\colhead{MJD}&\colhead{$I$}\\
\colhead{(1)}&\colhead{(2)}&\colhead{(3)}&\colhead{(4)}&\colhead{(5)}
&\colhead{(6)}&\colhead{(7)}&\colhead{(8)}
}
\startdata
27.3865 & 20.26 $\pm$ 0.16&  27.3946 &  19.06 $\pm$ 0.05  & 27.3784  & 18.43 $\pm$ 0.03   &27.3823 &  17.64 $\pm$ 0.03\\
28.3267 & 19.71 $\pm$ 0.10 & 28.3345 &  19.01 $\pm$ 0.06  & 28.3489  & 18.44 $\pm$ 0.04   &29.3473 &  17.63 $\pm$ 0.02\\
29.3514 & 19.94 $\pm$ 0.12 & 29.3592 &  19.08 $\pm$ 0.04  & 29.3749  & 18.44 $\pm$ 0.04   &30.3735 &  17.68 $\pm$ 0.03\\
30.3775 & 19.75 $\pm$ 0.09 & 30.3867 &  19.11 $\pm$ 0.05  & 30.4004  & 18.56 $\pm$ 0.04   &36.3600 &  17.54 $\pm$ 0.03\\
36.3641 & 20.05 $\pm$ 0.13 & 36.3719 &  19.11 $\pm$ 0.05  & 36.3860  & 18.35 $\pm$ 0.04   &38.4367 &  17.35 $\pm$ 0.04\\
38.4407 & 19.75 $\pm$ 0.18&  38.4499 &  18.86 $\pm$ 0.12  & 38.4317  & 18.14 $\pm$ 0.05   &73.3255 &  16.28 $\pm$ 0.02\\
73.3294 & 18.98 $\pm$ 0.15 & 73.3373 &  18.03 $\pm$ 0.06  & 73.3186  & 17.20 $\pm$ 0.05   &74.3874 &  15.79 $\pm$ 0.05\\
76.3644 & 17.43 $\pm$ 0.04 & 76.3698 &  16.64 $\pm $0.01  & 73.3452  & 17.35 $\pm$ 0.06   &76.3604 &  15.06 $\pm$ 0.01\\
77.2980 & 17.12 $\pm $0.02&  77.3033 &  16.27 $\pm$ 0.00  & 74.3834  & 17.00 $\pm$ 0.06   &77.2938 &  14.73 $\pm$ 0.01\\
77.4132 & 16.91 $\pm$ 0.02 & 77.4172 &  16.09 $\pm$ 0.01  & 76.3565  & 15.92 $\pm$ 0.01   &77.4099 &  14.51 $\pm$ 0.01\\
78.2467 & 17.69 $\pm$ 0.02 & 78.2519 &  16.80 $\pm$ 0.02  & 77.2894   &15.64 $\pm$ 0.01   &78.2417 &  15.09 $\pm$ 0.01\\
78.3157 & 17.69 $\pm$ 0.03&  78.3210 &  16.74 $\pm$ 0.02  & 77.3307  & 15.53 $\pm$ 0.01   &78.3103 &  15.16 $\pm$ 0.01\\
78.3901 & 17.59 $\pm$ 0.03 & 78.3957 &  16.65$ \pm$ 0.01  & 77.4282  & 15.46 $\pm$ 0.01   &78.4002 &  15.05 $\pm$ 0.01\\
78.4690&  17.20 $\pm$ 0.05&  78.4737 &  16.32 $\pm$ 0.01  & 77.4433  & 15.57 $\pm$ 0.01  & 78.4667 &  14.69 $\pm$ 0.01\\
79.2352 & 17.75 $\pm$ 0.02 & 79.2405 &  16.85$ \pm$ 0.01  & 77.4552   &15.69 $\pm$ 0.01  & 79.2325 &  15.25 $\pm$ 0.01\\
79.2906 & 17.83 $\pm$ 0.02 & 79.2959 &  16.89 $\pm$ 0.01  & 77.4640   &15.73 $\pm$ 0.01 &  79.2872 &  15.17 $\pm$ 0.01\\
79.3453 & 17.89 $\pm$ 0.03 & 79.3506 &  16.92 $\pm$ 0.01  & 77.4743   &15.73 $\pm$ 0.01  & 79.3417 &  15.20 $\pm$ 0.01\\
79.4146 & 18.12 $\pm$ 0.05 & 79.4200 &  17.16 $\pm$ 0.02 &  77.4836   &15.87 $\pm$ 0.01  & 79.4240 &  15.42 $\pm$ 0.01\\
80.2401 & 18.64 $\pm$ 0.06 & 80.2443 &  17.64 $\pm$ 0.02  & 77.4961   &15.83 $\pm$ 0.01  & 80.2371 &  15.84 $\pm$ 0.01\\
81.4688 & 18.61 $\pm $0.15 & 81.4727 &  17.70 $\pm$ 0.04  & 78.2328   &16.04 $\pm$ 0.01  & 81.4657 &  15.81 $\pm$ 0.01\\
85.3997 & 18.27 $\pm$ 0.05 & 85.4035 &  17.30 $\pm$ 0.01  & 78.2596   &16.09 $\pm$ 0.01  & 85.4075 &  15.60 $\pm$ 0.01\\
85.4220 & 18.29 $\pm$ 0.06 & 85.4262 &  17.26 $\pm$ 0.04  & 78.2753   &16.10 $\pm$ 0.01  & 85.4192 &  15.54 $\pm$ 0.01\\
86.2337 & 18.22 $\pm$ 0.03 & 86.2374 &  17.33 $\pm$ 0.01  & 78.2875  & 16.12 $\pm$ 0.01 &  86.2309 &  15.62 $\pm$ 0.01\\
88.3472 & 18.29 $\pm$ 0.09 & 88.3512 &  17.51 $\pm$ 0.05 & 78.3010   &16.12 $\pm$ 0.01  & 88.3445 &  15.73 $\pm$ 0.01\\
        &                &         &                &  78.3292  & 16.09 $\pm$ 0.01& &\\
        &               &          &                &  78.3445   &16.10 $\pm$ 0.01& &\\
        &               &           &               &  78.3578  & 16.02 $\pm$ 0.01 &&\\
        &               &           &               &  78.3758  & 15.96 $\pm$ 0.01& &\\
        &               &           &              &   78.4115  & 15.83 $\pm$ 0.01& &\\
        &               &           &              &   78.4202  & 15.80 $\pm$ 0.01 &&\\
        &               &           &              &   78.4293  & 15.76 $\pm$ 0.01 &&\\
        &               &           &              &   78.4393  & 15.71 $\pm$ 0.01& &\\
        &               &           &              &   78.4487  & 15.65 $\pm$ 0.01 &&\\
        &               &           &              &   78.4606  & 15.64 $\pm$ 0.02 &&\\
        &               &           &              &  78.4809   &15.60 $\pm$ 0.01 &&\\
        &               &           &              &   78.4911  & 15.62 $\pm$ 0.02 &&\\
        &               &            &             &   79.2265  & 16.11 $\pm$ 0.02 &&\\
        &               &            &             &   79.2470  & 16.09 $\pm$ 0.02& &\\
        &               &            &             &   79.2551  & 16.08 $\pm$ 0.02 &&\\
         &             &             &             &   79.2635   &16.08 $\pm$ 0.02& &\\
         &             &             &             &   79.2723   &16.11 $\pm$ 0.01& &\\
         &             &             &             &   79.2808  & 16.10 $\pm$ 0.01 &&\\
         &             &              &            &   79.3034  & 16.18 $\pm$ 0.02& &\\
          &             &             &             &  79.3115   &16.17 $\pm$ 0.02& &\\
          &             &             &            &   79.3197   &16.18 $\pm$ 0.03& &\\
          &            &              &            &   79.3281  & 16.16 $\pm$ 0.02& &\\
         &             &              &            &   79.3358  & 16.20 $\pm$ 0.02& &\\
         &             &              &            &   79.3629   &16.20 $\pm$ 0.02& &\\
          &            &              &             &  79.3711  & 16.25 $\pm$ 0.02& &\\
         &             &              &             &  79.3791   &16.26 $\pm$ 0.02 &&\\
         &             &              &             &  79.3873   &16.32 $\pm$ 0.02& &\\
         &             &              &             &  79.3966  & 16.35 $\pm$ 0.02& &\\
         &             &              &              & 79.4056  & 16.39 $\pm$ 0.01& &\\
         &             &              &              & 81.4570  & 16.93 $\pm$ 0.03& &\\
         &             &               &             & 81.4805  & 16.89 $\pm$ 0.03& &\\
         &             &              &              & 85.3936  & 16.62 $\pm$ 0.03& &\\
         &             &              &              & 85.4129  & 16.54 $\pm$ 0.02 &&\\
         &             &               &             & 86.2249   &16.61 $\pm$ 0.03& &\\
         &             &              &             &  86.2446  & 16.57 $\pm$ 0.02 &&\\
         &              &             &             &  86.3557  & 16.58 $\pm$ 0.01& &\\
         &             &              &              & 86.3637  & 16.60 $\pm$ 0.01 &&\\
         &             &              &              & 88.3384   &16.75 $\pm$ 0.01& &\\
\enddata
\tablecomments{MJD is JD-2454000}
\end{deluxetable}


==> table2.tex <==
\begin{deluxetable}{lrlrlr}
\singlespace
\tablecolumns{6}
\tablecaption{\bf Near-IR Data \label{TAB_2}}
\tabletypesize{\footnotesize}
\tablehead{
\colhead{MJD}&\colhead{$J$}&\colhead{MJD}&\colhead{$H$}&
\colhead{MJD}&\colhead{$K$}\\
\colhead{(1)}&\colhead{(2)}&\colhead{(3)}&\colhead{(4)}&\colhead{(5)}
&\colhead{(6)}
}
\startdata
 979.5576 & 17.24 $\pm$ 0.11 &  979.5627 & 16.49 $\pm$   0.14  & 979.5666 &  15.31 $\pm $  0.19 \\
 980.6155 & 17.24 $\pm$   0.07 &  980.6206 & 16.32 $\pm$   0.09 &  980.6258  & 15.47 $\pm $  0.15 \\
 985.5727 & 17.27 $\pm $  0.05 &  985.5778 & 16.18 $\pm$   0.04 &  985.5828 &  15.69 $\pm$   0.16 \\
 988.5093 & 16.93 $\pm$   0.04 &  988.5152 & 16.08 $\pm$   0.04 &  988.5203 &  15.08 $\pm$   0.08 \\
 989.5445 & 17.14 $\pm$   0.11 &  989.5495 & 16.32 $\pm$   0.10 &  989.5547 &  15.26 $\pm$   0.10 \\
1002.5165 & 17.13 $\pm $  0.07 & 1002.5215 & 16.05 $\pm $  0.07 & 1002.5267 &  14.95 $\pm$   0.11 \\
1003.5560 & 16.92 $\pm$   0.04 & 1003.5593 & 16.17 $\pm$   0.06 & 1003.5627 &  15.14 $\pm$   0.07 \\
1007.5171 & 16.80 $\pm $  0.04 & 1007.5222 & 15.84 $\pm$   0.05 & 1007.5273 &  15.02 $\pm $  0.08 \\
1009.5209 & 16.34 $\pm $  0.03 & 1009.5261 & 15.37 $\pm$   0.04 & 1009.5312  & 14.52 $\pm $  0.07 \\
1010.5058 & 16.25 $\pm$   0.02 & 1010.5112 & 15.35 $\pm$   0.02 & 1010.5164 &  14.32 $\pm$   0.04 \\
1011.5281 & 16.54 $\pm$   0.03 & 1011.5332 & 15.54 $\pm$   0.02 & 1011.5382 &  14.56 $\pm$   0.05 \\
1022.4241 & 16.18 $\pm $  0.03 & 1022.4287 & 15.05 $\pm $  0.03 & 1022.4331 &  14.06 $\pm$   0.05 \\
1054.3726 & 15.56 $\pm $  0.02 & 1054.3766 & 14.47 $\pm$   0.02 & 1054.3805 &  13.43 $\pm$   0.03 \\
1063.4242 & 15.02 $\pm $  0.01 & 1063.4270 & 13.94 $\pm$   0.01 & 1063.4303 &  12.93 $\pm$   0.01 \\
1065.4003 & 15.43 $\pm$   0.02 & 1065.4036 & 14.30 $\pm $  0.02 & 1065.4069 &  13.28 $\pm$   0.02 \\
1066.3946 & 14.78 $\pm$   0.01 & 1066.3972 & 13.67 $\pm$   0.01 & 1066.4000 &  12.75 $\pm$   0.01 \\
1067.3747 & 15.23 $\pm $  0.02 & 1067.3775 & 14.19 $\pm $  0.02 & 1067.3801 &  13.19 $\pm $  0.02 \\
1068.3753 & 15.10 $\pm$   0.01 & 1068.3779 & 14.02 $\pm$   0.01 & 1068.3808 &  12.93 $\pm$   0.02 \\
1069.3394 & 14.90 $\pm $  0.01 & 1069.3423 & 13.83 $\pm$   0.01 & 1069.3452 &  12.85 $\pm $  0.01 \\
1070.4049 & 14.80 $\pm$   0.01 & 1070.4075 & 13.75 $\pm$   0.01 & 1070.4104 &  12.74 $\pm$   0.01 \\
1071.3871 & 14.86 $\pm$   0.01 & 1071.3899 & 13.79 $\pm$   0.01 & 1071.3927 &  12.77 $\pm$   0.02 \\
1075.3512 & 14.36 $\pm$   0.01 & 1075.3556 & 13.30 $\pm $  0.01 & 1075.3589 &  12.29 $\pm$   0.01 \\
1076.3372 & 13.89 $\pm$   0.01 & 1076.3398 & 12.88 $\pm $  0.01 & 1076.3424 &  11.92 $\pm$   0.01 \\
1077.3914 & 13.28 $\pm$   0.01 & 1077.3944 & 12.28 $\pm$   0.01 & 1077.3972 &  11.38 $\pm$   0.01 \\
1077.4339 & 13.29 $\pm$   0.01 & 1077.4368 & 12.34 $\pm$   0.01 & 1077.4397  & 11.47 $\pm $  0.01 \\
1077.4425 & 13.33 $\pm$   0.01 & 1077.4452 & 12.39 $\pm$   0.01 & 1077.4478 &  11.53 $\pm $  0.01 \\
1077.4593 & 13.48 $\pm$   0.01 & 1077.4620 & 12.54 $\pm$   0.01 & 1077.4695  & 11.60 $\pm $  0.01 \\
1077.4847 & 13.63 $\pm$   0.01 & 1077.4876 & 12.63 $\pm $  0.01 & 1077.4904 &  11.69 $\pm$   0.01 \\
1077.4932 & 13.60 $\pm$   0.01 & 1077.4960 & 12.59 $\pm$   0.01 & 1077.4986  & 11.65 $\pm$   0.01 \\
1077.5018 & 13.56 $\pm$   0.01 & 1077.5046 &  12.57 $\pm$   0.01 & 1077.5075 &  11.69 $\pm $  0.01 \\
1077.5120 & 13.61 $\pm$   0.01 & 1077.5150 &  12.63 $\pm$   0.01 & 1077.5180 &  11.68 $\pm $  0.01 \\
1077.5237 & 13.64 $\pm$   0.01 & 1077.5265 &  12.65 $\pm$   0.01 & 1077.5293 &  11.66 $\pm$   0.01 \\
1077.5324 & 13.60 $\pm$   0.01 & 1077.5383 &  12.57 $\pm$   0.01 & 1077.5411 &  11.62 $\pm$   0.01 \\
1077.5511 & 13.58 $\pm$   0.01 & 1077.5542 &  12.56 $\pm$   0.01 & 1077.5571 &  11.67 $\pm $  0.01 \\
1077.5601 & 13.64 $\pm$   0.01 & 1077.5627 &  12.62 $\pm$   0.01 & 1077.5656 &  11.64 $\pm$   0.01 \\
1077.5699 & 13.61 $\pm$   0.01 & 1077.5728 &  12.62 $\pm$   0.01 & 1077.5754 &  11.66 $\pm$   0.01 \\
1077.5782 & 13.56 $\pm$   0.01 & 1077.5812 &  12.52 $\pm$   0.01 & 1077.5840 &  11.64 $\pm$   0.01 \\
1081.3752 & 14.38 $\pm$   0.01 & 1081.3789 &  13.27 $\pm $  0.01 & 1081.3818 &  12.18 $\pm $  0.01 \\
1081.3847 & 14.41 $\pm$   0.01 & 1081.3875 &  13.23 $\pm$   0.01 & 1081.4284 &  12.19 $\pm$   0.01 \\
1081.4230 & 14.38 $\pm$   0.01 & 1081.4258 &  13.24 $\pm$   0.01 & 1081.4366 &  12.18 $\pm$   0.01 \\
1081.4312 & 14.35 $\pm$   0.01 & 1081.4338  & 13.23 $\pm$   0.01 & 1081.4451 &  12.19 $\pm $  0.01 \\
1081.4394 & 14.38 $\pm$   0.01 & 1081.4423 &  13.23 $\pm$   0.01 & 1081.4533 &  12.18 $\pm$   0.01 \\
1081.4478 & 14.31 $\pm$   0.01 & 1081.4506 &  13.26 $\pm$   0.01 & 1081.4619  & 12.20 $\pm $  0.01 \\
1081.4560 & 14.33 $\pm$   0.01 & 1081.4591 &  13.21 $\pm$   0.01 & 1081.4822 &  12.16 $\pm $  0.01 \\
1081.4754 & 14.32 $\pm $  0.01 & 1081.4795 &  13.25 $\pm $  0.01 & 1081.4903 &  12.23 $\pm $  0.01 \\
1081.4850 & 14.35 $\pm $  0.01 & 1081.4876 &  13.24 $\pm$   0.01 & 1081.5048 &  12.22 $\pm $  0.01 \\
1081.4958 & 14.40 $\pm$   0.01 & 1081.4931 &  13.19 $\pm$   0.01 & 1081.5133 &  12.19 $\pm$   0.01 \\
1081.5075 & 14.32 $\pm$   0.01 & 1081.5102 &  13.22 $\pm$   0.01 & 1082.3279 &  12.17 $\pm $  0.01 \\
1082.3221 & 14.20 $\pm$   0.01 & 1082.3250 &  13.14 $\pm$   0.01 & 1082.3365  & 12.15 $\pm$   0.01 \\
1082.3310 & 14.24 $\pm $  0.01 & 1082.3338 &  13.12 $\pm$   0.01 & 1082.3555 &  12.13 $\pm$   0.01 \\
1082.3499 & 14.26 $\pm$   0.01 & 1082.3527 &  13.14 $\pm$   0.01 & 1082.3639 &  12.15 $\pm$   0.01 \\
1082.3586 & 14.26 $\pm$   0.01 & 1082.3613 &  13.12 $\pm$   0.01 & 1082.3734 &  12.15 $\pm$   0.01 \\
1082.3672 & 14.23 $\pm$   0.01 & 1082.3706 &  13.13 $\pm$   0.01 & 1082.3818 &  12.17 $\pm $  0.01 \\
1082.3763 & 14.24 $\pm$   0.01 & 1082.3790 &  13.16 $\pm$   0.01 & 1083.4604 &  12.27 $\pm $  0.01 \\
1083.4550 & 14.38 $\pm$   0.01 & 1083.4577 &  13.31 $\pm$   0.01  \\
\enddata
\tablecomments{MJD is JD-2453000}
\end{deluxetable}


==> table3.tex <==
\begin{deluxetable}{lrr}
\singlespace
\tablecolumns{3}
\tablecaption{\bf Polarization Data in $R$ band\label{TAB_3}}
\tabletypesize{\footnotesize}
\tablehead{
\colhead{MJD}&\colhead{$p$,\%}&\colhead{$\Theta^\circ$} \\
\colhead{(1)}&\colhead{(2)}&\colhead{(3)}
}
\startdata
77.3307 &  32.7 $\pm$ 1.0  & 149.5 $\pm$  0.8\\
77.4282 &  27.7 $\pm$ 1.4  & 152.2 $\pm$  1.3\\
77.4433 &  25.9 $\pm$ 1.6 &  153.8 $\pm $ 1.8\\
77.4552 &  23.8 $\pm$ 2.1 &  156.6 $\pm$  2.4\\
77.4640 &  23.4 $\pm$ 2.1 &  153.7 $\pm$  2.5\\
77.4743 &  24.2 $\pm$ 2.2 &  153.8 $\pm$  2.6\\
77.4836 &  22.6 $\pm $2.5 &  153.2 $\pm$  3.1\\
77.4961 &  19.0 $\pm$ 2.5 &  150.7 $\pm$  3.9\\
78.2328 &   8.1 $\pm$ 1.3 &  116.1 $\pm$  4.7\\
78.2596 &  10.0 $\pm$ 1.5 &  110.8 $\pm$  4.2\\
78.2753 &  11.8 $\pm$ 1.5  & 119.4 $\pm$  3.6\\
78.2875 &   7.4 $\pm$ 1.5 &  105.7 $\pm$  5.8\\
78.3010  & 10.7 $\pm$ 1.7 &  104.9 $\pm$  4.6\\
78.3292  & 13.8 $\pm$ 1.7 &  110.9 $\pm$  3.5\\
78.3445  &  7.6 $\pm$ 1.4 &  130.8 $\pm $ 5.4\\
78.3578  & 11.9 $\pm$ 1.4 &  125.0 $\pm$  3.4\\
78.3758  & 12.9 $\pm$ 1.5 &  117.3 $\pm$  3.2\\
78.4115 &  16.3$ \pm$ 1.9 &  117.7 $\pm $ 3.3\\
78.4202 &  16.7 $\pm$ 2.0 &  125.9 $\pm $ 3.4\\
78.4293 &  15.7 $\pm$ 1.9 &  120.5 $\pm$  3.5\\
78.4393 &  17.1 $\pm$ 2.0 &  124.7 $\pm $ 3.3\\
78.4487 &  17.7 $\pm$ 1.9 &  126.3$ \pm$  3.1\\
78.4606 &  19.4 $\pm$ 1.9 &  121.1 $\pm$  2.8\\
78.4809  & 19.4 $\pm$ 2.1 &  124.9 $\pm$  3.0\\
78.4911  & 17.6 $\pm$ 2.1 &  128.5 $\pm$  3.4\\
79.2265  & 10.3 $\pm$ 1.5 &  126.1 $\pm$  4.2\\
79.2470  & 10.9 $\pm$ 1.3 &  123.2 $\pm $ 3.5\\
79.2551 &  12.9 $\pm$ 1.4 &  121.3 $\pm$  3.1\\
79.2635 &  12.6 $\pm$ 1.4 &  125.0 $\pm $ 3.2\\
79.2723 &  10.9 $\pm$ 1.6 &  122.8 $\pm $ 4.1\\
79.2808 &  10.7 $\pm $1.7 &  122.7 $\pm$  4.5\\
79.3034 &   6.7 $\pm$ 1.8 &  122.3 $\pm$  7.6\\
79.3115  &  9.1 $\pm$ 1.8 &  114.3 $\pm$  5.7\\
79.3197 &   9.2 $\pm$ 1.8 &  124.0 $\pm$  5.9\\
79.3281 &  10.8 $\pm$ 1.8  & 120.2 $\pm$  4.9\\
79.3358 &    7.5 $\pm$ 1.9 &  117.9 $\pm $ 7.2\\
79.3629 &    8.3 $\pm $2.2 &  125.8 $\pm$  7.7\\
79.3711 &    9.1 $\pm$ 2.1 &  111.8 $\pm$  6.5\\
79.3791 &     7.7 $\pm$ 2.1&   111.6 $\pm$  7.8\\
79.3873 &    7.3 $\pm$ 2.4&   120.0 $\pm$  9.4\\
79.3966 &    5.4 $\pm$ 2.5 &  119.2 $\pm$ 13.3\\
79.4056 &    5.4 $\pm$ 2.8 &  127.6 $\pm$ 14.8\\
81.4570 &   15.1 $\pm$ 5.5 &  128.4 $\pm$ 10.3\\
81.4805 &   14.9 $\pm$ 4.6 &  129.9 $\pm$  8.9\\
85.3936 &    2.6 $\pm$ 2.5 &  137.6 $\pm$ 27.4\\
85.4129 &    1.6 $\pm$ 2.4 &  158.0 $\pm$ 43.3\\
86.2249 &    4.2 $\pm$ 2.2 &  126.2 $\pm$ 14.9\\
86.2446 &    6.6 $\pm$ 2.1 &  107.8 $\pm$  9.0\\
86.3557  &   4.7 $\pm$ 2.7  &  92.2 $\pm$ 16.6\\
86.3637 &    8.0 $\pm$ 4.3 &  112.8 $\pm$ 15.6\\
88.3384 &  10.6 $\pm$ 5.3  &  75.4 $\pm$ 14.4 \\
\enddata
\tablecomments{MJD is JD-2454000}
\end{deluxetable}

